Token-Level Uncertainty-Aware Objective for Language Model Post-Training

In the current work, we connect token-level uncertainty in causal language modeling to two types of training objectives: 1) masked maximum likelihood (MLE), 2) self-distillation. We show that masked MLE is effective in reducing epistemic uncertainty, and serve as an effective token-level automatic curriculum learning technique. However, masked MLE is prone to overfitting and requires self-distillation regularization to improve or maintain performance on out-of-distribution tasks. We demonstrate significant performance gain via the proposed training objective - combined masked MLE and self-distillation - across multiple architectures (Gemma, LLaMA, Phi) and datasets (Alpaca, ShareGPT, GSM8K), mitigating overfitting while maintaining adaptability during post-training. Our findings suggest that uncertainty-aware training provides an effective mechanism for enhancing language model training.

==> latex/eval.tex <==

In practice, for both AlpacaEval and MT-Bench benchmarks, the model generations were evaluated head-to-head to the generations from the baseline, adjusted for both length and positional biases. Given the scale of the experiments, we opted to use \texttt{Qwen/Qwen2.5-7B-Instruct} model as the judge, which in Oct. 2024 was the highest ranked judge model on Judge Arena that is smaller than 50B in parameter size. Additionally, to improve evaluation granularity, we differentiate between single-turn, multi-turn and combined win rate of MT-Bench. For tasks with ground truth metrics such as IF-Eval and GSM8K, we report both the raw performance metrics as well as the normalized the model performance (\texttt{(model - baseline) / baseline}).

==> latex/perf.tex <==
In this section, we provide additional information on evaluation procedure as well as  experimental results that highlight both in-distribution and out-of-distribution performance gains of the various training paradigms discussed in the current manuscript.

\subsection{Evaluation Detail}\label{sec:appx:perf:eval}
For freeform QA tasks such as AlpacaEval and MT-Bench benchmarks, the experiment generations (models trained with objectives other than MLE) were evaluated head-to-head to the generations from the baseline (model trained with MLE), adjusted for both length and positional biases. Given the scale of the experiments, we opted to use \texttt{Qwen/Qwen2.5-7B-Instruct} model as the judge, which in Oct. 2024 was the highest ranked judge model on Judge Arena that is smaller than 50B in parameter size. Additionally, to improve evaluation granularity, we differentiate between single-turn, multi-turn and combined win rate of MT-Bench. For tasks with ground truth metrics such as IF-Eval and GSM8K, we report both the raw performance metrics as well as the normalized the model performance (\texttt{(model - baseline) / baseline}).
